Neural functional a posteriori error estimates

We propose a new loss function for supervised and physics-informed training of neural networks and operators that incorporates a posteriori error estimate. More specifically, during the training stage, the neural network learns additional physical fields that lead to rigorous error majorants after a computationally cheap postprocessing stage. Theoretical results are based upon the theory of functional a posteriori error estimates, which allows for the systematic construction of such loss functions for a diverse class of practically relevant partial differential equations. From the numerical side, we demonstrate on a series of elliptic problems that for a variety of architectures and approaches (physics-informed neural networks, physics-informed neural operators, neural operators, and classical architectures in the regression and physics-informed settings), we can reach better or comparable accuracy and in addition to that cheaply recover high-quality upper bounds on the error after training.

==> figures/tables/equation_description.tex <==
\begin{tabular}{lccc}
\toprule
Shortcut & $a(x)$ & $b(x)$ & Equation \\
$\text{smooth}_{b}$ & smooth & $\surd$ & \eqref{eq:elliptic_1}\\
$\text{disc}_{o}$ & discontinuous & $\times$ & \eqref{eq:elliptic_3}\\
$\text{disc}_{b}$ & discontinuous & $\surd$ & \eqref{eq:elliptic_4}\\
$\text{smooth}_{o}$ & smooth & $\times$ & \eqref{eq:elliptic_6}\\
\bottomrule
\end{tabular}

==> figures/tables/parameters_unsupervised_learning_for_2D.tex <==
\begin{center}
\begin{tabular}{lcccc}
\toprule
& fSNO & ChebNO & DilResNet & UNet \\
\# parameters& $116 \times 10^{3}$ & $116\times 10^{3}$ & $326 \times 10^{3}$ & $248 \times 10^{3}$ \\
\bottomrule
\end{tabular}
\end{center}

==> figures/unsupervised_result_eq.tex <==
\begin{tabular}{crrrrrr}
\toprule
{equation} &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
\midrule
\eqref{eq:elliptic_1_1D} &               0.011 &              0.015 &                           0.019 &                          0.034 &                           0.827 &                          0.855 \\
\eqref{eq:elliptic_2_1D} &               0.010 &              0.015 &                           0.015 &                          0.032 &                           0.822 &                          0.854 \\
\eqref{eq:elliptic_3_1D} &               0.033 &              0.034 &                           0.037 &                          0.039 &                           0.791 &                          0.792 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_result_eq_2D.tex <==
% \begin{tabular}{crrrrrr}
% \toprule
% {equation} &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\

% \midrule
% \eqref{eq:elliptic_1} &                0.013 &               0.014 &                            0.027 &                           0.036 &                            0.847 &                           0.788 \\
% \eqref{eq:elliptic_3} &                0.019 &               0.019 &                            0.023 &                           0.024 &                            0.837 &                           0.827 \\
% \eqref{eq:elliptic_4} &                0.029 &               0.029 &                            0.049 &                           0.052 &                            0.906 &                           0.901 \\
% \eqref{eq:elliptic_6} &                0.013 &               0.015 &                            0.027 &                           0.038 &                            0.855 &                           0.810 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{crrrrrr}
\toprule
{equation} &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
\midrule
\eqref{eq:elliptic_1} &                0.011 &               0.013 &                            0.022 &                           0.029 &                            0.849 &                           0.816 \\
\eqref{eq:elliptic_3} &                0.018 &               0.019 &                            0.023 &                           0.024 &                            0.809 &                           0.831 \\
\eqref{eq:elliptic_4} &                0.027 &               0.031 &                            0.046 &                           0.053 &                            0.899 &                           0.890 \\
\eqref{eq:elliptic_6} &                0.012 &               0.013 &                            0.024 &                           0.030 &                            0.847 &                           0.822 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_result_eq_2D_add.tex <==



\begin{tabular}{crrrrrr}
\toprule
{$J$} &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\

\midrule
5 &                0.012 &               0.014 &                            0.025 &                           0.037 &                            0.854 &                           0.791 \\
6 &                0.013 &               0.014 &                            0.031 &                           0.040 &                            0.847 &                           0.835 \\
7 &                0.023 &               0.025 &                            0.055 &                           0.061 &                            0.850 &                           0.842 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_result_model.tex <==
\begin{tabular}{crrrrrr}
\toprule
Architecture &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
\midrule
fSNO      &               0.014 &              0.016 &                           0.022 &                          0.026 &                           0.828 &                          0.861 \\
ChebNO    &               0.016 &              0.018 &                           0.026 &                          0.029 &                           0.835 &                          0.853 \\
DilResNet &               0.017 &              0.018 &                           0.018 &                          0.022 &                           0.771 &                          0.777 \\
UNet      &               0.023 &              0.033 &                           0.028 &                          0.061 &                           0.821 &                          0.844 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_result_model_2D.tex <==
% \begin{tabular}{crrrrrr}
% \toprule
% Architecture &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
% \midrule
% fSNO         &                0.016 &               0.017 &                           0.028 &                          0.035 &                           0.864 &                          0.836 \\
% ChebNO       &                0.017 &               0.018 &                           0.030 &                          0.037 &                           0.882 &                          0.853 \\
% DilResNet    &                0.012 &               0.012 &                           0.015 &                          0.019 &                           0.845 &                          0.811 \\
% UNet         &                0.029 &               0.030 &                           0.051 &                          0.060 &                           0.862 &                          0.828 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{crrrrrr}
\toprule
Architecture &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
\midrule
fSNO         &                0.012 &               0.013 &                           0.024 &                          0.031 &                           0.844 &                          0.821 \\
ChebNO       &                0.013 &               0.015 &                           0.028 &                          0.034 &                           0.858 &                          0.847 \\
DilResNet    &                0.008 &               0.009 &                           0.015 &                          0.018 &                           0.823 &                          0.771 \\
UNet         &                0.012 &               0.014 &                           0.023 &                          0.035 &                           0.872 &                          0.823 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_result_model_2D_add.tex <==


\begin{tabular}{crrrrrr}
\toprule
Architecture &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
\midrule
fSNO         &                0.015 &               0.017 &                           0.035 &                          0.045 &                           0.853 &                          0.826 \\
ChebNO       &                0.016 &               0.018 &                           0.039 &                          0.049 &                           0.842 &                          0.818 \\
DilResNet    &                0.009 &               0.010 &                           0.021 &                          0.026 &                           0.837 &                          0.808 \\
UNet         &                0.025 &               0.027 &                           0.054 &                          0.064 &                           0.870 &                          0.838 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_result_trsize.tex <==
\begin{tabular}{crrrrrr}
\toprule
$N_{\text{train}}$ &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
\midrule
200      &               0.036 &              0.048 &                           0.060 &                          0.102 &                           0.840 &                          0.839 \\
400      &               0.026 &              0.033 &                           0.041 &                          0.066 &                           0.825 &                          0.841 \\
600      &               0.023 &              0.029 &                           0.032 &                          0.052 &                           0.810 &                          0.839 \\
800      &               0.021 &              0.026 &                           0.030 &                          0.047 &                           0.823 &                          0.842 \\
1000     &               0.019 &              0.023 &                           0.026 &                          0.040 &                           0.823 &                          0.845 \\
1200     &               0.018 &              0.021 &                           0.023 &                          0.035 &                           0.814 &                          0.834 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_result_trsize_2D.tex <==
% \begin{tabular}{crrrrrr}
% \toprule
% $N_{\text{train}}$ &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
% \midrule
% 200      &                0.038 &               0.042 &                            0.064 &                           0.085 &                            0.884 &                           0.845 \\
% 400      &                0.025 &               0.027 &                            0.045 &                           0.059 &                            0.893 &                           0.860 \\
% 600      &                0.026 &               0.027 &                            0.043 &                           0.054 &                            0.885 &                           0.849 \\
% 800      &                0.020 &               0.021 &                            0.036 &                           0.044 &                            0.874 &                           0.844 \\
% 1000     &                0.019 &               0.020 &                            0.033 &                           0.041 &                            0.868 &                           0.843 \\
% 1200     &                0.018 &               0.019 &                            0.031 &                           0.038 &                            0.861 &                           0.831 \\
% \bottomrule
% \end{tabular}


\begin{tabular}{crrrrrr}
\toprule
$N_{\text{train}}$ &  $E_{\text{train}}$ &  $E_{\text{test}}$ &  $E^{\text{ub}}_{\text{train}}$ &  $E^{\text{ub}}_{\text{test}}$ &  $R^{\text{ub}}_{\text{train}}$ &  $R^{\text{ub}}_{\text{test}}$ \\
\midrule
200      &                0.038 &               0.042 &                            0.065 &                           0.084 &                            0.885 &                           0.854 \\
400      &                0.025 &               0.028 &                            0.045 &                           0.059 &                            0.892 &                           0.862 \\
600      &                0.026 &               0.028 &                            0.043 &                           0.054 &                            0.884 &                           0.860 \\
800      &                0.020 &               0.022 &                            0.036 &                           0.045 &                            0.876 &                           0.854 \\
1000     &                0.019 &               0.021 &                            0.033 &                           0.042 &                            0.870 &                           0.851 \\
1200     &                0.018 &               0.020 &                            0.031 &                           0.038 &                            0.858 &                           0.844 \\
1400     &                0.018 &               0.019 &                            0.030 &                           0.036 &                            0.857 &                           0.846 \\
1600     &                0.018 &               0.019 &                            0.029 &                           0.035 &                            0.855 &                           0.842 \\
1800     &                0.018 &               0.019 &                            0.029 &                           0.034 &                            0.851 &                           0.840 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_test_all_models_2D.tex <==
\begin{tabular}{cllllllll}
\toprule
$N_{\text{train}}$  &                \multicolumn{2}{c}{fSNO} & \multicolumn{2}{c}{ChebNO} & \multicolumn{2}{c}{DilResNet} & \multicolumn{2}{c}{UNet} \\
{} &  $E_{\text{test}}$ &     $E^{\text{up}}_{\text{test}}$ &  $E_{\text{test}}$ &     $E^{\text{up}}_{\text{test}}$ &          $E_{\text{test}}$ &     $E^{\text{up}}_{\text{test}}$ &                        $E_{\text{test}}$ &    $E^{\text{up}}_{\text{test}}$ \\

\midrule
200  &  0.041  &  0.078  &  0.042 &  0.081 &  0.029 &  0.063 &         0.055 &  0.115 \\
400  &  0.027 &  0.057 & 0.029 &  0.059 &  0.019 &   0.039 &   0.038 &    0.080 \\
600   &  0.023 &    0.048 &  0.024 &  0.050 & 0.015 &  0.030 &   0.048 &    0.085 \\
800   &   0.020 &   0.042 &  0.021 &  0.044 &  0.014 &  0.025 &      0.034 &    0.068 \\
1000    &    0.018 &     0.038 & 0.020 &  0.040 &  0.013 &            0.022 &    0.033 &      0.066 \\
1200     &   0.018 &      0.036 &   0.018 &                               0.036 &     0.012 &    0.019 &     0.032 &    0.063 \\
1400     &      0.017  &   0.033 &   0.018 &   0.034 &   0.012 &  0.017 &     0.031 &   0.059 \\
1600    &     0.016 &    0.030 &  0.016 &  0.032 &  0.012 &            0.016 &    0.031 &      0.060 \\
1800  &   0.015 &   0.029 &    0.016 &  0.031 &   0.012 &  0.015 &     0.033 &     0.062 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_unet.tex <==
\begin{tabular}{cllllllll}
\toprule
$N_{\text{train}}$  &                \multicolumn{2}{c}{fSNO} & \multicolumn{2}{c}{ChebNO} & \multicolumn{2}{c}{DilResNet} & \multicolumn{2}{c}{UNet} \\
{} &  $E_{\text{train}}$ &     $E_{\text{test}}$ &  $E_{\text{train}}$ &     $E_{\text{test}}$ &          $E_{\text{train}}$ &     $E_{\text{test}}$ &                        $E_{\text{train}}$ &    $E_{\text{test}}$ \\
\midrule
200                &               0.028 &  0.036 &                       0.035 &                 0.044 &                                      0.031 &                 0.041 &                        0.05 &  0.071 \\
400                &                0.02 &                 0.025 &                       0.025 &                 0.029 &                                       0.02 &                 0.024 &                       0.038 &                0.055 \\
600                &               0.019 &                 0.022 &                        0.02 &                 0.023 &                                      0.019 &                 0.021 &                       0.033 &                0.049 \\
800                &               0.017 &                 0.019 &                       0.019 &                 0.021 &                       0.018 &                  0.02 &                       0.031 &                0.044 \\
1000               &               0.015 &                 0.016 &                       0.017 &  0.018 &                                      0.017 &                 0.019 &                       0.028 &                 0.04 \\
1200               &               0.014 &                 0.016 &                       0.016 &  0.018 &                                      0.017 &  0.018 &                       0.023 &                0.033 \\
\bottomrule
\end{tabular}

==> figures/unsupervised_unet_2D.tex <==
% \begin{tabular}{cllllllll}
% \toprule
% $N_{\text{train}}$  &                \multicolumn{2}{c}{fSNO} & \multicolumn{2}{c}{ChebNO} & \multicolumn{2}{c}{DilResNet} & \multicolumn{2}{c}{UNet} \\
% {} &  $E_{\text{train}}$ &     $E_{\text{test}}$ &  $E_{\text{train}}$ &     $E_{\text{test}}$ &          $E_{\text{train}}$ &     $E_{\text{test}}$ &                        $E_{\text{train}}$ &    $E_{\text{test}}$ \\
% \midrule
% 200                &                 0.037 &                  0.040 &                                       0.040 &                 0.042 &                                      0.025 &                 0.029 &                       0.048 &              0.055 \\
% 400                &                 0.025 &                 0.027 &                       0.026 &                 0.028 &                                      0.017 &  0.018 &                       0.031 &              0.037 \\
% 600                &                 0.021 &                 0.022 &                                      0.022 &                 0.024 &                                      0.014 &                 0.015 &                       0.046 &              0.047 \\
% 800                &  0.018 &                  0.020 &                                      0.019 &                 0.021 &                       0.013 &                 0.014 &                        0.031 &              0.032 \\
% 1000               &                 0.017 &  0.018 &                                      0.017 &                 0.019 &                                      0.012 &  0.013 &                        0.030 &              0.031 \\
% 1200               &                 0.016 &                 0.017 &                                      0.017 &  0.018 &                                      0.012 &                 0.012 &                       0.029 &               0.030 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{cllllllll}
\toprule
$N_{\text{train}}$  &                \multicolumn{2}{c}{fSNO} & \multicolumn{2}{c}{ChebNO} & \multicolumn{2}{c}{DilResNet} & \multicolumn{2}{c}{UNet} \\
{} &  $E_{\text{train}}$ &     $E^{\text{up}}_{\text{train}}$ &  $E_{\text{train}}$ &     $E^{\text{up}}_{\text{train}}$ &          $E_{\text{train}}$ &     $E^{\text{up}}_{\text{train}}$ &                        $E_{\text{train}}$ &    $E^{\text{up}}_{\text{train}}$ \\

\midrule
200                &  0.037 &    0.062 &    0.039 &      0.067 &       0.025 &         0.049 &  0.049 &    0.080 \\
400                &  0.024 &    0.044 &    0.027 &      0.047 &       0.017 &         0.030 &  0.031 &    0.059 \\
600                &  0.021 &    0.038 &    0.022 &      0.040 &       0.014 &         0.024 &  0.045 &    0.072 \\
800                &  0.018 &    0.032 &    0.019 &      0.035 &       0.013 &         0.020 &  0.031 &    0.056 \\
1000               &  0.017 &    0.029 &    0.018 &      0.032 &       0.013 &         0.018 &  0.030 &    0.054 \\
1200               &  0.016 &    0.028 &    0.017 &      0.029 &       0.012 &         0.015 &  0.029 &    0.052 \\
1400               &  0.015 &    0.026 &    0.016 &      0.028 &       0.012 &         0.014 &  0.028 &    0.051 \\
1600               &  0.015 &    0.025 &    0.015 &      0.027 &       0.012 &         0.013 &  0.029 &    0.052 \\
1800               &  0.014 &    0.024 &    0.015 &      0.026 &       0.011 &         0.012 &  0.030 &    0.053 \\
\bottomrule
\end{tabular}
